S$^3$R: Fast and Faithful RL Rollouts via Self-Sparse Speculative Decoding

Fast rollout generation for long-context reinforcement learning with verifiable rewards (RLVR) requires reducing KV-cache traffic without changing the response groups used for policy optimization. In our profiled RLVR workloads, attention accounts for 72--76\% of autoregressive decoding kernel time. Sparse attention reduces these reads, but sampling directly from a sparse policy changes the response groups used for learning. For group-relative optimization, we show that even exact response-wise reweighting does not generally recover the expected dense-policy update because the advantage of each response depends on the rewards of other group members. We propose Self-Sparse Speculative Rollouts (S$^3$R). It uses sparse attention to propose tokens, then generates responses through full-attention verification and exact speculative sampling. Drafting and verification share the same policy parameter, eliminating the need to train or update a separate drafter. The resulting response groups follow the dense-policy distribution. Under S$^3$R, we characterize speedup conditions and the costs of drafting and verification. We found that dense verification still requires the complete historical KV cache. A KV-aware scheduler therefore limits KV-cache repeated offloading and restoration while maintaining rollout parallelism. % OR thrashing In a matched ablation with an aggressive sparse drafting budget, S$^3$R maintains stable training while direct sparse sampling with training-side correction becomes unstable. On long-context mathematical reasoning, S$^3$R achieves $1.39\times~1.35\times$ the end-to-end training throughput of autoregressive rollouts on Qwen3 model, with comparable task performance.

==> appendices/sparse_self_speculation_measurements.tex <==
% Integrated from figs/why_ssrl_2. Reported numerical results are unchanged.
% Input within Appendix app:why-ssrl, after its component analysis and profiles.

\subsection{Controlled budget--acceptance trade-off}
\label{app:why-ssrl-budget}

We vary the sparse budget while measuring both acceptance and throughput
to test the trade-off in Section~\ref{sec:efficiency-runtime}.
These measurements use real mathematical continuations and complete
GPU-work windows, complementing the component profiles above.

\paragraph{Models and inputs.}
Qwen3-1.7B and Qwen3-8B each use their frozen DAPO step-60 checkpoint,
BF16, two H100 80GB GPUs, TP$=2$, $k=6$, asynchronous CPU scheduling,
and SparseAttn with a minimum
budget of 192 tokens. Sparse decoding and the full-attention AR reference
use the same rollout engine (Appendix~\ref{app:ssrl-implementation}). Each run
starts with 64 resident requests at context length 8192. We sweep configured
budgets $s_{\mathrm{cfg}}\in\{0.03,0.05,0.10,0.20,0.35,0.50\}$;
here K denotes 1024 tokens.

For each model, the first 192 distinct dense-AR continuations of DAPO
prompts that reach context 8192 without EOS form three disjoint bundles of
64 inputs, fixed across AR and all budgets. All runs use temperature one
and engine RNG seed 330. EOS is
disabled during timing, and the workload is conditional on survival to 8K.
Each configuration has 18 sparse runs and three AR references; the six
ratios within a bundle share one AR denominator. The primary configurations
are 1.7B/Graph160 and 8B/Graph640, with 8B/Graph160 as an additional control.

\paragraph{Timing and useful progress.}
Timing starts after at least 50 ready iterations, once mean committed
context reaches 8256, then covers at least 256 further committed tokens per
request on average. Sparse endpoints follow complete verification and commitment.
No requests enter or leave the active set during these windows, and no KV pages are offloaded. CUDA is drained
at both endpoints, with no added internal synchronization; the terminal
drain is included and the terminal TP barrier excluded. We use the larger
TP-rank time and require paired AR/sparse endpoint mean contexts to differ
by at most 32 tokens.

For committed output counts $Y$ and elapsed times $T$, each paired speedup is
\begin{equation}
 \eta_j=\frac{Y_{\mathrm{SS},j}/T_{\mathrm{SS},j}}
                  {Y_{\mathrm{AR},j}/T_{\mathrm{AR},j}}.
 \label{eq:why-ssrl-window-speedup}
\end{equation}
Progress counts accepted drafts plus one correction or bonus token per
completed request round, with $\tau_j=1+k\alpha_j$
(Appendix~\ref{app:why-ssrl-cost}). Effective $s_j$ is logical draft KV
reads divided by the corresponding full KV volume, including minimum-budget,
rounding, and appended-token effects. It is measured independently of
acceptance and time and does not measure physical HBM traffic.

\paragraph{Measured budget trade-off.}
Higher acceptance need not yield higher throughput
(Figure~\ref{fig:why-ssrl-budget-overlay}). Increasing the budget from 0.05 to
0.50 raises representative acceptance from 0.795 to 0.958 for 1.7B and
from 0.804 to 0.967 for 8B, while median speedup falls from
$1.533\times$ to $1.094\times$ and from $1.370\times$ to $1.058\times$.
Reducing the budget from 0.05 to 0.03 also lowers speedup, to $1.469\times$
and $1.307\times$. Both accepted progress and execution cost therefore matter.
The sampled 0.05--0.10 region performs well without resolving a unique
optimum.
Each plotted estimate uses the measured acceptance and effective budget
of the run with median speedup at that budget.

\begin{figure}[tbp]
 \centering
 \begin{subfigure}[t]{0.48\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figs/why_ssrl_2/figs/subfigs/budget_tradeoff_1_7b.pdf}
  \caption{Qwen3-1.7B.}\label{fig:why-ssrl-budget-overlay-1-7b}
 \end{subfigure}\hfill
 \begin{subfigure}[t]{0.48\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figs/why_ssrl_2/figs/subfigs/budget_tradeoff_8b.pdf}
  \caption{Qwen3-8B.}\label{fig:why-ssrl-budget-overlay-8b}
 \end{subfigure}
 \caption{Measured and estimated speedup across sparse budgets for
 (\subref{fig:why-ssrl-budget-overlay-1-7b}) Qwen3-1.7B and
 (\subref{fig:why-ssrl-budget-overlay-8b}) Qwen3-8B at $B=64$, initial $S=8$K, and $k=6$.
 Orange diamonds denote held-out medians; blue stars denote RL observations
 at an effective draft KV-read ratio of 5\%.}
 \label{fig:why-ssrl-budget-overlay}
\end{figure}

\subsection{Calibration of the component approximation}
\label{app:why-ssrl-calibration}

We normalize Eq.~\ref{eq:why-ssrl-mixed-latency} by the two-component AR
approximation, with attention fraction and projection scaling
\begin{equation}
 \rho=\frac{T_{\mathrm{Attn}}(M)}
 {T_{\mathrm{GEMM}}(B)+T_{\mathrm{Attn}}(M)},\qquad
 g_k=\frac{T_{\mathrm{GEMM}}\!\left(\frac{2k+1}{k+1}B\right)}
 {T_{\mathrm{GEMM}}(B)}.
 \label{eq:why-ssrl-calibration-anchors}
\end{equation}
The normalized round cost and ideal speedup are then
\begin{equation}
 D_0(s)=(k+1)g_k(1-\rho)+(1+ks)\rho,\qquad
 \eta_0=\frac{\tau}{D_0(s)}.
 \label{eq:why-ssrl-normalized-cost}
\end{equation}
We fix $\rho$ and $g_k$ from independent AR profiles before fitting.
The attention fraction uses $(B,S)=(64,8\mathrm{K})$ and excludes other
kernels and communication. For $g_k$, we interpolate projection costs at
$B=64$ and 128, measured at $S=4$K, to $B=118.86$. This is a proxy for
projection scaling in a mixed draft--verify pass at $S=8$K.

\paragraph{Calibration and held-out budgets.}
We fit the residual $\tau_j/\eta_j-D_0(s_j)$ on budgets 0.03, 0.10,
0.35, and 0.50 (12 equally weighted observations), holding out 0.05 and
0.20 (six observations). A linear residual replaces a constant only if
leave-one-calibration-budget-out cost RMSE improves by at least 20\% and
bundle-specific slopes agree in sign, with positive, nondecreasing cost on
$s\in[0.025,0.52]$. All three configurations select a constant $\delta$:
\begin{equation}
 \widehat\eta(\alpha,s)=\frac{1+k\alpha}{D_0(s)+\delta},\qquad
 \delta=\frac{1}{12}\sum_{j\in\mathcal C}
 \left[\frac{\tau_j}{\eta_j}-D_0(s_j)\right],
 \label{eq:why-ssrl-calibrated-speedup}
\end{equation}
where $\mathcal C$ is the calibration set and $k=6$. Held-out budgets and
RL timings enter neither fitting nor selection. The model takes measured
acceptance as input, with break-even condition
$\alpha>[D_0(s)+\delta-1]/k$.

\paragraph{Conditional speedup surfaces.}
Figure~\ref{fig:why-ssrl-surfaces} plots
Eq.~\ref{eq:why-ssrl-calibrated-speedup} over effective KV-read ratio $s$
and accepted-prefix fraction $\alpha$, using the primary configurations
in Table~\ref{tab:why-ssrl-fit}. At fixed $s$, higher acceptance increases
useful progress; at fixed acceptance, a larger budget raises attention cost.
The observations follow a workload-dependent $\alpha(s)$ trajectory, so
higher acceptance can accompany lower speedup. All measured points exceed
$1\times$; the break-even contour and low-acceptance region remain
conditional extrapolations beyond this trajectory.
The color scale saturates outside $0.5\times$--$2\times$.

\begin{figure}[tbp]
 \centering
 \newlength{\ssrlSurfacePanelWidth}
 \setlength{\ssrlSurfacePanelWidth}{0.43\linewidth}
 \begin{subfigure}[t]{\ssrlSurfacePanelWidth}
  \vspace{0pt}\centering
  \includegraphics[width=\linewidth]{figs/why_ssrl_2/figs/subfigs/surface_1_7b.pdf}
  \caption{Qwen3-1.7B.}\label{fig:why-ssrl-surface-1-7b}
 \end{subfigure}\hfill
 \begin{subfigure}[t]{\ssrlSurfacePanelWidth}
  \vspace{0pt}\centering
  \includegraphics[width=\linewidth]{figs/why_ssrl_2/figs/subfigs/surface_8b.pdf}
  \caption{Qwen3-8B.}\label{fig:why-ssrl-surface-8b}
 \end{subfigure}\hfill
 \begin{minipage}[t]{0.10\linewidth}
  \vspace{0pt}\centering
  \includegraphics[height=0.83\ssrlSurfacePanelWidth]{figs/why_ssrl_2/figs/subfigs/speedup_colorbar.pdf}
 \end{minipage}
 \par\medskip
 \includegraphics[width=0.90\linewidth]{figs/why_ssrl_2/figs/subfigs/surface_legend.pdf}
 \caption{Estimated speedup as a function of effective draft KV-read ratio and acceptance for
 (\subref{fig:why-ssrl-surface-1-7b}) Qwen3-1.7B and
 (\subref{fig:why-ssrl-surface-8b}) Qwen3-8B.
 Circles and diamonds denote calibration and held-out observations; the dark contour marks break-even.
 Blue stars denote RL observations at effective draft KV-read ratio $s=0.05$.}
 \label{fig:why-ssrl-surfaces}
\end{figure}

\begin{table}[t]
 \centering\small\setlength{\tabcolsep}{4pt}
 \input{figs/why_ssrl_2/tables/fit_summary}
 \caption{Component parameters, fitted residual, and errors on the six
 held-out observations. Ideal and Cal. denote predictions before and after
 calibration; MAPE and max. are mean and maximum absolute percentage errors.}
 \label{tab:why-ssrl-fit}
\end{table}

\paragraph{Execution costs beyond the approximation.}
Calibration reduces held-out MAPE from 84.61\% to 0.80\% for 1.7B and
from 63.03\% to 0.68\% for primary 8B. The residual combines execution
overhead with error in the projection-scaling proxy and AR normalizer.
Timed batches include synchronized drafting, verification, and no-forward
stalls that can expose unfinished GPU work. Sparse selection, communication,
and asynchronous waits further separate elapsed time from component costs.
The residual does not identify these contributions individually.

\subsection{Execution and workload sensitivity}
\label{app:why-ssrl-sensitivity}

\paragraph{Prediction versus measurement.}
Figure~\ref{fig:why-ssrl-prediction-parity} shows agreement between
calibrated and measured speedup along the observed budget trajectories.
It includes all 54 calibration and held-out observations across the three
configurations; Table~\ref{tab:why-ssrl-fit} isolates the held-out errors.

\paragraph{Execution configurations.}
Both 8B configurations show the same budget trade-off, with speedup
approaching $1\times$ at higher budgets
(Figure~\ref{fig:why-ssrl-execution-configurations}). KV capacity and
background CPU activity also differ, so this comparison does not isolate
CUDA Graph effects.

\begin{figure}[tbp]
 \centering
 \begin{subfigure}[t]{0.48\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figs/why_ssrl_2/figs/subfigs/prediction_parity.pdf}
  \caption{Prediction versus measurement.}\label{fig:why-ssrl-prediction-parity}
 \end{subfigure}\hfill
 \begin{subfigure}[t]{0.48\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figs/why_ssrl_2/figs/subfigs/execution_configurations_8b.pdf}
  \caption{8B execution configurations.}\label{fig:why-ssrl-execution-configurations}
 \end{subfigure}
 \caption{Execution sensitivity.
 (\subref{fig:why-ssrl-prediction-parity}) Predicted versus measured speedup across 54 profiling runs,
 with the diagonal denoting equality;
 (\subref{fig:why-ssrl-execution-configurations}) median speedup for the two Qwen3-8B execution configurations.}
 \label{fig:why-ssrl-execution}
\end{figure}

\paragraph{Changing batch or context.}
Table~\ref{tab:why-ssrl-states} varies batch or context at budget 0.05
using primary 1.7B and 8B/Graph160, with one input bundle per state,
excluded from fitting. EOS is disabled, so some 16K contexts extend beyond
an earlier EOS. Speedup varies with inference state; these diagnostics
do not validate transferring the $(64,8\mathrm{K})$ calibration unchanged.

\begin{table}[t]
 \centering\small
 \input{figs/why_ssrl_2/tables/state_diagnostics}
 \caption{Batch/context diagnostics at budget 0.05. Each row reports one
 paired throughput measurement without independent replication.}
 \label{tab:why-ssrl-states}
\end{table}

\subsection{Comparison with real RL rollouts}
\label{app:why-ssrl-rl}

We compare four paired 1.7B RL steps and three paired 8B steps with the
frozen local models. Each step generates eight responses per prompt for
256 prompts across four TP2 replicas, using full verification, CPU KV
offloading, and maximum concurrency 256 per replica. The AR baseline uses
vLLM, with prompt identities matched across methods; sampled outputs
and counts can differ.
The effective draft KV-read ratio for these RL observations is $s=0.05$.
% The authors confirmed the effective ratio on 2026-09-17; the previous
% 0.03/proxy wording was a stale placeholder.

\paragraph{RL markers in the surfaces and budget curves.}
Figures~\ref{fig:why-ssrl-budget-overlay} and
\ref{fig:why-ssrl-surfaces} show three steps per model. For 1.7B,
steps 72, 73, and 75 (a/b/c) are sampled uniformly without replacement from
steps 72--75 using seed 42; all four enter the aggregate comparison below.
For 8B, a/b/c show all available steps, 71/72/73. Stars use measured
acceptance and speedup at their effective ratio $s=0.05$.

\paragraph{Generation-throughput comparison.}
RL speedup compares aggregate output throughputs,
\begin{equation}
 \eta_{\mathrm{RL}}=
 \frac{\sum_t Y_{\mathrm{SS},t}/\sum_t T_{\mathrm{SS},t}}
      {\sum_t Y_{\mathrm{dense},t}/\sum_t T_{\mathrm{dense},t}}.
 \label{eq:why-ssrl-rl-speedup}
\end{equation}
Here $T$ is generation wall time, excluding RL optimization. These short
comparisons are separate from the main training runs. Aggregate acceptance
is total accepted drafts divided by total proposed drafts.

The measured aggregate speedups are $1.558\times$ for 1.7B and
$1.491\times$ for 8B, at acceptance 0.757 and 0.771. The primary local
models estimate $1.518\times$ and $1.352\times$, respectively
($-2.59\%$ and $-9.32\%$ relative to measurement). Applying the 8B control
calibration to the same three steps gives $1.321\times$ ($-11.41\%$).
% Numerical estimates retained as requested on 2026-09-17. This revision
% corrects the RL-marker ratio description only; no numerical refit is performed.
These runs support RL acceleration, but differences in workload, offloading,
AR baseline, and timing scope mean that local held-out errors do not quantify
RL prediction accuracy.


==> appendices/why_sparse_self_speculation.bak.tex <==
% Paper-ready appendix section for the systems rationale of \modelname.
% Bibliography keys match the DBLP entries used in the main text.
% Expected packages: graphicx.

\section{Why Self-Sparse Speculative Decoding for RL Rollouts?}
\label{app:why-ssrl}

This appendix supports the latency discussion in
Section~\ref{sec:efficiency-runtime}. We decompose projection and
attention costs, derive a feasibility condition, and profile the components
across rollout workloads. Controlled budget sweeps in
Appendix~\ref{app:why-ssrl-budget} then measure accepted progress and
throughput together. Calibration, workload diagnostics, and separate RL
observations examine the scope of these local measurements.

\subsection{Latency decomposition for self-sparse speculative decoding}
\label{app:why-ssrl-cost}

We extend the serialized latency accounting in
Eq.~\ref{eq:efficiency-sd-accounting} by separating projection work from
historical KV reads at locally fixed active batch size $B$ and mean cached
context length $S$. For complete rounds, let $\alpha$ be the mean fraction
of the $k$ draft tokens accepted; then $\tau=1+k\alpha\in[1,k+1]$.

Let $T_{\mathrm{GEMM}}(B)$ cover QKVO, FFN, and LM-head work, and let
$T_{\mathrm{Attn}}(M)$ cover attention at aggregate KV volume
$M\propto B\cdot S$. The shared-weight drafter retains projection work but
reads a fraction $s\in(0,1]$ of the historical KV. We approximate
bandwidth-bound attention latency as linear in $M$. Verification processes
the $k$ drafts plus the preceding round's final token, whose dense KV is
not yet cached. Assuming $k+1\ll S$ and shared historical reads across
these $(k+1)B$ queries gives
\begin{equation}
\begin{aligned}
 T_p&=T_{\mathrm{GEMM}}(B)+T_{\mathrm{Attn}}(M),\\
 T_q&=T_{\mathrm{GEMM}}(B)+sT_{\mathrm{Attn}}(M),\\
 T_V&=T_{\mathrm{GEMM}}((k+1)B)+T_{\mathrm{Attn}}(M).
\end{aligned}
\label{eq:why-ssrl-sparse-stages}
\end{equation}
Projection latency need not scale linearly with $B$ because small batches
reuse weights. Larger batches can increase $T_V/T_p$, whereas longer
contexts at fixed $B$ push it toward one
\citep{sadhukhan2025magicdec,DBLP:journals/corr/abs-2606-18967}.

Shared weights also permit draft and verification queries in one forward.
With requests evenly staggered across $k$ draft stages and one verification
stage~\citep[Sections~3.2--3.3]{DBLP:journals/corr/abs-2512-01278},
each iteration has $kB/(k+1)$ single-query drafts and $B/(k+1)$
verifications of $k+1$ queries each. This yields $(2k+1)B/(k+1)$ queries
and $(ks+1)M/(k+1)$ effective KV reads per iteration. Each request
completes a round in $k+1$ iterations, so the mixed-stage cost per output
token is
\begin{equation}
 \frac{T_{\mathrm{mix}}}{\tau}
 =\frac{k+1}{\tau}\left[
 T_{\mathrm{GEMM}}\!\left(\frac{2k+1}{k+1}B\right)
 +T_{\mathrm{Attn}}\!\left(\frac{ks+1}{k+1}M\right)\right].
 \label{eq:why-ssrl-mixed-latency}
\end{equation}
By linearity, the attention term becomes $(ks+1)T_{\mathrm{Attn}}(M)/\tau$.

At full acceptance, $\tau=k+1$ maximizes output per round for fixed
$(B,S,s,k)$. Comparing Eq.~\ref{eq:why-ssrl-mixed-latency} with the AR
latency $T_p$ gives the ideal mixed-stage feasibility condition
\begin{equation}
 k(1-s)T_{\mathrm{Attn}}(M)
 >(k+1)\left[
 T_{\mathrm{GEMM}}\!\left(\frac{2k+1}{k+1}B\right)
 -T_{\mathrm{GEMM}}(B)\right].
 \label{eq:why-ssrl-full-acceptance}
\end{equation}
The left-hand side is the attention saving; the right-hand side is the
projection overhead from mixing draft and verification queries. If the
condition fails, no acceptance rate yields a speedup in this component
model. Observed acceleration also depends on actual acceptance and costs
beyond this approximation, examined in
Appendix~\ref{app:why-ssrl-calibration}.

\subsection{Component profiling setup}
\label{app:why-ssrl-setup}

We use $B$ for the active batch on one tensor-parallel (TP) rollout replica,
$S$ for the cached context length per request, and $N_{\mathrm{KV}}=B\cdot S$ for aggregate live
KV tokens in the fixed-length workloads. We use $1\mathrm{K}=1024$ tokens
for both context lengths and aggregate KV counts. Table~\ref{tab:why-ssrl-setup}
summarizes the common setting. Appendix~\ref{app:why-ssrl-e2} reports
acceptance thresholds in terms of $\alpha$, using $\tau=1+k\alpha$ from
Appendix~\ref{app:why-ssrl-cost}.

\begin{table}[t]
\centering
\small
\caption{Common setting for Appendices~\ref{app:why-ssrl-e1} and~\ref{app:why-ssrl-e2}.}
\label{tab:why-ssrl-setup}
\begin{tabular}{ll}
\hline
Item & Setting \\
\hline
Model & Qwen3-8B, DAPO step-60 checkpoint \\
Hardware & $2\times$NVIDIA H100 80GB HBM3 \\
Parallelism & one rollout-engine replica, TP${=}2$ \\
Precision & BF16 \\
Workload & equal-length synthetic prompts, fixed concurrency, ignore EOS \\
Sampling & temperature 0 (deterministic systems workload) \\
AR baseline & ordinary AR with full attention \\
Sparse draft & Pillar attention, ratio 0.05, minimum 192 tokens \\
Speculation & draft length $k=6$, exact full-model verification \\
\hline
\end{tabular}
\end{table}

We instrument scheduler iterations and model components with NVTX and collect
CUDA kernel traces using Nsight Systems. Attribution runs execute eagerly so
that the Python-level component ranges are visible. The profiles in
Appendix~\ref{app:why-ssrl-e1} use 50 ready-state warm-up iterations;
those in Appendix~\ref{app:why-ssrl-e2} use eight ready-state warm-up
iterations and one capture-settle iteration. Both record 20 measured
iterations. GPU component times are normalized per measured scheduler
iteration and per TP rank. For Appendix~\ref{app:why-ssrl-e1}, we assign
each classified kernel to its finest stable range and normalize component
shares by the sum of \emph{non-collective} GPU-kernel times. This excludes
topology-dependent TP collectives while retaining all memory traffic within
attention kernels. The attention profile in Appendix~\ref{app:why-ssrl-e2}
includes both draft and verification attention over all 20 scheduler states,
including two no-forward stall states. These profiles describe GPU work per
iteration; they do not normalize for differences in output length.

For the acceptance thresholds in Appendix~\ref{app:why-ssrl-e2}, $T_p$,
$T_q$, and $T_V$ are separately measured scheduler intervals, including CPU
time exposed around each GPU forward. Their sum $kT_q+T_V$ estimates sequential
stage costs and excludes no-forward stalls and cross-request phase mixing.
The synchronized workload does not isolate the scheduling mechanisms described in
Appendix~\ref{app:why-ssrl-cost}. Its thresholds are therefore
conditional on the measured stage costs; realized rollout speedup requires
matched end-to-end timing.

\subsection{Attention cost under rollout workloads}
\label{app:why-ssrl-e1}

We sweep $B\in\{1,4,16,32,64,128,256\}$ and
$S\in\{1,2,4,8,16,24,32\}\mathrm{K}$, subject to the measured KV-capacity
limit. This gives 35 feasible grid points.
We additionally profile $(B,S)=(8,2\mathrm{K})$ and $(2,4\mathrm{K})$, yielding
37 formal attribution traces in total.  The two added points complete the four
rollout-tail coordinates analyzed by EfficientRollout
~\citep{DBLP:journals/corr/abs-2606-18967}.

We group kernels into FFN, QKV and output projections (QKVO), attention, LM
head, and Other.  Other contains normalization, RoPE/KV append, elementwise,
embedding, sampling, and remaining scheduler GPU kernels.  Table~
\ref{tab:why-ssrl-e1-breakdown} first reproduces the small-$N_{\mathrm{KV}}$ rollout-tail
coordinates and then holds $B=16$ while increasing $S$.  Each component entry
is latency in milliseconds followed by its share of non-collective GPU-kernel
latency.

\begin{table*}[t]
\centering
\setlength{\tabcolsep}{5.5pt}
\caption{Decomposition of ordinary full-attention AR decoding.  Entries are
ms (percentage of the non-collective GPU-kernel total); TP collectives are
excluded from all columns and from the normalization.  The upper panel matches
the $(S,B)$ coordinates used in the rollout-tail analysis of
EfficientRollout~\citep{DBLP:journals/corr/abs-2606-18967}; the lower panel exposes the
long-context transition on our workload.}
\label{tab:why-ssrl-e1-breakdown}
\begin{tabular}{@{}rrrrrrrr@{}}
\hline
$N_{\mathrm{KV}}$ & $S$ & $B$ & Attention & FFN & QKVO & LM head & Others \\
\hline
8K   & 2K  & 4   & 0.96 (19.4\%)  & 2.18 (43.8\%) & 0.83 (16.6\%) & 0.21 (4.1\%) & 0.80 (16.1\%) \\
8K   & 4K  & 2   & 0.93 (18.8\%)  & 2.18 (44.2\%) & 0.82 (16.6\%) & 0.20 (4.2\%) & 0.80 (16.2\%) \\
8K   & 8K  & 1   & 0.98 (19.8\%)  & 2.17 (43.7\%) & 0.82 (16.5\%) & 0.20 (4.1\%) & 0.79 (16.0\%) \\
16K  & 2K  & 8   & 1.16 (22.4\%)  & 2.19 (42.1\%) & 0.83 (16.0\%) & 0.21 (4.0\%) & 0.81 (15.6\%) \\
\hline
64K  & 4K  & 16  & 2.34 (36.2\%)  & 2.24 (34.6\%) & 0.85 (13.2\%) & 0.21 (3.3\%) & 0.82 (12.7\%) \\
128K & 8K  & 16  & 3.85 (48.4\%)  & 2.23 (28.1\%) & 0.85 (10.7\%) & 0.21 (2.6\%) & 0.82 (10.3\%) \\
256K & 16K & 16  & 6.85 (62.4\%)  & 2.24 (20.4\%) & 0.85 (7.8\%)  & 0.21 (1.9\%) & 0.82 (7.5\%) \\
512K & 32K & 16  & 12.93 (75.8\%) & 2.24 (13.2\%) & 0.85 (5.0\%)  & 0.21 (1.2\%) & 0.82 (4.8\%) \\
512K & 16K & 32  & 12.98 (75.1\%) & 2.37 (13.7\%) & 0.87 (5.1\%)  & 0.21 (1.2\%) & 0.84 (4.9\%) \\
512K & 8K  & 64  & 13.11 (76.2\%) & 2.23 (13.0\%) & 0.76 (4.4\%)  & 0.21 (1.2\%) & 0.89 (5.2\%) \\
512K & 4K  & 128 & 13.07 (75.2\%) & 2.32 (13.4\%) & 0.80 (4.6\%)  & 0.22 (1.3\%) & 0.97 (5.6\%) \\
512K & 2K  & 256 & 13.44 (72.3\%) & 2.73 (14.7\%) & 0.99 (5.4\%)  & 0.24 (1.3\%) & 1.18 (6.3\%) \\
\hline
\end{tabular}
\end{table*}

At the four rollout-tail points, FFN, QKVO, and LM-head projections together
account for 62.1--65.0\% of non-collective kernel latency, while attention
accounts for 18.8--22.4\%.  This agrees qualitatively with the projection-bound
tail regime reported by EfficientRollout, despite differences in model,
hardware, TP degree, and measurement method.  The conclusion reverses as the
live KV volume grows: at $B=16$, attention rises from 2.34 ms at $S=4$K to
12.93 ms at $S=32$K, while FFN remains approximately 2.24 ms.

Figure~\ref{fig:why-ssrl-e1-ratio} shows the complete feasible grid as the
ratio of attention to FFN latency.  The ratio is below one in the small-$N_{\mathrm{KV}}$
tail, crosses one as aggregate live KV grows, and reaches 4.92--5.88 across the
feasible factorizations of $N_{\mathrm{KV}}=512$K.  Factoring the same $N_{\mathrm{KV}}$ differently also
gives similar ratios: 0.43--0.45 at $N_{\mathrm{KV}}=8$K, 0.97--1.12 at $N_{\mathrm{KV}}=64$K,
1.64--1.81 at $N_{\mathrm{KV}}=128$K, and 2.72--3.14 at $N_{\mathrm{KV}}=256$K.  Therefore neither $B$
nor $S$ alone describes the bottleneck.  For full-attention single-token
decoding in this range, their product $N_{\mathrm{KV}}=B\cdot S$ is the useful first-order
indicator of when KV-cache attention overtakes FFN.

\begin{figure}[t]
\centering
\includegraphics[width=0.68\linewidth]{figs/why_ssrl/e1_attention_ffn_heatmap.pdf}
\caption{Attention-to-FFN kernel latency ratio for full-attention AR decoding
across batch sizes and context lengths.
The black contour marks equal latency; hatched cells exceed the measured KV-capacity limit.}
\label{fig:why-ssrl-e1-ratio}
\end{figure}

\subsection{Drafting and verification costs}
\label{app:why-ssrl-e2}

We profile attention and draft--verify stage costs at eight feasible points
with $B\in\{16,32,64\}$ and $S\in\{4,8,16\}$K. Every reported value is the
median of three fresh profiling processes. These component measurements
complement the complete-window throughput measurements in
Appendix~\ref{app:why-ssrl-budget}.

\paragraph{Attention reduction.}
Table~\ref{tab:why-ssrl-e2-attention} compares attention GPU time in
full-attention AR and \modelname. The latter includes sparse drafting and
full-attention verification, averaged over the measured scheduler window.

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\caption{Attention profile.  Times are median NVTX GPU projections in ms per
measured scheduler iteration per TP rank over three processes.  \modelname includes
both sparse draft attention and full verification attention and is normalized
over all 20 scheduler states, including two no-forward stall states.  These are
component times, not per-output-token or end-to-end iteration times.}
\label{tab:why-ssrl-e2-attention}
\begin{tabular}{@{}rrrrrrr@{}}
\hline
$B$ & $S$ & $N_{\mathrm{KV}}$ & Full attention & \modelname attention & Saved & Reduction \\
\hline
16 & 4K  & 64K  & 2.31 & 1.42 & 0.88 & 38.3\% \\
16 & 8K  & 128K & 3.83 & 1.89 & 1.94 & 50.6\% \\
16 & 16K & 256K & 6.82 & 2.79 & 4.04 & 59.2\% \\
32 & 4K  & 128K & 3.80 & 1.96 & 1.84 & 48.5\% \\
32 & 8K  & 256K & 6.83 & 2.85 & 3.98 & 58.3\% \\
32 & 16K & 512K & 12.91 & 4.68 & 8.23 & 63.7\% \\
64 & 4K  & 256K & 6.91 & 2.90 & 4.02 & 58.1\% \\
64 & 8K  & 512K & 13.02 & 4.79 & 8.23 & 63.2\% \\
\hline
\end{tabular}
\end{table*}

The per-iteration attention saving rises from 0.88 ms at $N_{\mathrm{KV}}=64$K to
8.23 ms at $N_{\mathrm{KV}}=512$K, where the reduction reaches 63.2--63.7\%.
Similar savings across different $(B,S)$ factorizations of the same $N_{\mathrm{KV}}$
support aggregate live KV as an indicator of the available attention saving.

\paragraph{Draft and verification costs.}
For the measured stage costs, comparing $kT_q+T_V$ with the equal-output
AR cost $\tau T_p=(1+k\alpha)T_p$ gives the break-even acceptance
\begin{equation}
 \alpha_{\mathrm{BE}}^{\mathrm{stage}}
 =\frac{1}{k}\left(\frac{kT_q+T_V}{T_p}-1\right).
 \label{eq:why-ssrl-stage-threshold}
\end{equation}
Acceleration under this accounting requires
$\alpha>\alpha_{\mathrm{BE}}^{\mathrm{stage}}$.
Table~\ref{tab:why-ssrl-e2-stages} reports this threshold for $k=6$,
alongside the draft subtotal $6T_q$, verification cost $T_V$, and their
sum. The AR reference is $7T_p$, corresponding to full acceptance.

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\caption{Block-equivalent stage-time accounting for $k=6$.  AR max block is
$7T_p$, Draft subtotal is $6T_q$, and \modelname block is
$6T_q+T_V$.  Latencies (ms) are constructed
from medians over three process-level stage medians after aligning TP ranks and
selecting the critical rank.  Full AR and draft use CUDA Graphs; verification
is eager because its query batch $7B$ exceeds the capture bound. The
constructed block cost excludes no-forward stalls and cross-request phase
mixing (Appendix~\ref{app:why-ssrl-setup}).}
\label{tab:why-ssrl-e2-stages}
\begin{tabular}{@{}rrrrrrrr@{}}
\hline
$B$ & $S$ & $N_{\mathrm{KV}}$ & AR max block & Draft subtotal & Verify & \modelname block & $\alpha_{\mathrm{BE}}^{\mathrm{stage}}$ \\
\hline
16 & 4K  & 64K  & 54.42 & 40.06 & 28.06 & 68.12 & $>100\%$ \\
16 & 8K  & 128K & 65.55 & 39.15 & 27.97 & 67.12 & $>100\%$ \\
16 & 16K & 256K & 88.51 & 42.38 & 28.10 & 70.48 & 76.2\% \\
32 & 4K  & 128K & 66.70 & 40.89 & 29.03 & 69.92 & $>100\%$ \\
32 & 8K  & 256K & 88.12 & 43.01 & 26.86 & 69.87 & 75.8\% \\
32 & 16K & 512K & 133.18 & 43.73 & 28.56 & 72.29 & 46.7\% \\
64 & 4K  & 256K & 87.22 & 42.05 & 27.96 & 70.01 & 77.0\% \\
64 & 8K  & 512K & 129.85 & 42.51 & 26.68 & 69.19 & 45.5\% \\
\hline
\end{tabular}
\end{table*}

Under this accounting, even full acceptance cannot amortize the measured
stage costs at $N_{\mathrm{KV}}=64$K--128K. The threshold decreases to 75.8--77.0\% at
$N_{\mathrm{KV}}=256$K and 45.5--46.7\% at $N_{\mathrm{KV}}=512$K, while verification remains
substantial at 26.68--29.03 ms. Larger live KV volume thus creates more room
to amortize drafting and verification. These thresholds use separately
measured sequential stages; Eq.~\ref{eq:why-ssrl-full-acceptance} instead
assumes mixed-stage execution. The stage thresholds are not pooled with
the complete-window throughput measurements below.

\input{appendices/sparse_self_speculation_measurements}


==> figs/estimated_speed_up/alpha_s_1_7b_figure.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/supporting_systems/estimated_speed_up/fig_alpha_s_speedup_1_7b.pdf}
  \caption{Rollout-anchored conditional speedup estimate for Qwen3-1.7B with $k=6$.
  The effective cost scale is calibrated to four paired post-warmup Offload and AR
  rollout steps, using output tokens per generation wall time across four TP=2 replicas.
  The aggregate measured speedup is $1.558\times$ at nominal budget $s_{\mathrm{cfg}}=0.03$;
  the acceptance coordinate uses aggregated accepted/proposed counters.
  Purple squares show the four step coordinates and the filled diamond is their aggregate anchor.
  The inset displays each measured speedup and the estimate from the surface calibrated using all
  four steps; this agreement is not independent validation.
  Gray circles show 19 measured checkpoint acceptance fractions at nominal budget 0.05 under a
  different rollout workload, without paired AR speedup measurements.
  Budget dependence is an assumed linear cost scenario with slope $\beta=6$;
  no 1.7B component profiling or matched budget sweep is used to determine this slope.
  The surface estimates rollout throughput gains under these assumptions, not fixed-state GPU latency.}
  \label{fig:alpha-s-speedup-1-7b}
\end{figure}


==> figs/estimated_speed_up/alpha_s_calibrated_figure.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/supporting_systems/estimated_speed_up/fig_alpha_s_speedup_calibrated.pdf}
  \caption{Profiling-anchored conditional speedup estimate for Qwen3-8B at $k=6$,
  $B=64$, and nominal $S=8$K on two H100 GPUs with TP=2.
  The ideal component model uses measured AR attention and GEMM costs and an interpolated
  pure-AR query-scaling proxy. An additive normalized round-cost correction is calibrated
  to the median of three scheduler-window estimates from
  Appendix~\ref{app:why-ssrl-e2} at effective KV-read ratio
  $s\approx0.05046$ (brown diamond). These estimates reconstruct equal committed progress
  from KV growth between identical verification phases and use CPU scheduler interval sums;
  they are not synchronized GPU wall-time measurements. The calibration anchor is not an
  independent validation point. The dependence on $s$ retains the ideal linear-cost assumption.
  Gray circles show twelve measured checkpoint acceptance fractions at nominal budget
  $s_{\mathrm{cfg}}=0.05$; their variable-length rollouts provide an acceptance reference,
  rather than matched-state speedup measurements. The purple square is a separate paired
  Offload versus AR rollout comparison over three RL steps, with nominal budget
  $s_{\mathrm{cfg}}=0.03$ and logged acceptance proxy $\alpha\approx0.771$.
  Its runtime speedup of $1.49\times$ is the ratio of output tokens per generation wall time.
  Its variable batch/context and timing scope differ from the local profiling surface;
  it is a cross-workload reference, not a matched-state validation point.
  Both callouts distinguish runtime-derived speedups from the surface estimates.}
  \label{fig:alpha-s-speedup-calibrated}
\end{figure}


==> figs/estimated_speed_up/alpha_s_prediction_figure.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/supporting_systems/estimated_speed_up/fig_alpha_s_speedup_prediction.pdf}
  \caption{Conditional speedup predicted by the balanced self-speculative component model
  at $k=6$, $B=64$, and $S=8$K for Qwen3-8B on two H100 GPUs with TP=2.
  Measured full-AR attention and GEMM times determine $\rho=0.803$;
  the mixed-query GEMM multiplier $g_k=1.036$ is estimated from neighboring pure-AR
  query batches. The model assumes linear attention cost and shared verification KV reads,
  and excludes other kernels, TP collectives, and exposed scheduling overhead.
  Purple markers show measured accepted-prefix fractions from ten variable-length checkpoint
  rollouts, positioned at their nominal budget $s_{\mathrm{cfg}}=0.05$.
  Their aggregate effective KV-read ratios are unavailable; the markers indicate an observed
  acceptance regime, rather than matched-state measurements of the background speedup.
  The black contour marks the predicted break-even boundary.}
  \label{fig:alpha-s-speedup-prediction}
\end{figure}


==> figs/estimated_speed_up/estimated_speedup_section.tex <==
% Include from the paper directory with:
% \input{figures/supporting_systems/estimated_speed_up/estimated_speedup_section}
% Requires amsmath, amssymb, graphicx, and booktabs.
% Self-contained section: no document environment or references to external labels.

\section{From Latency Decomposition to Empirically Anchored Speedup Surfaces}
\label{sec:estimated-speedup}

We use a conditional cost model to examine when sparse self-speculation can
accelerate generation. The model connects the fraction of accepted draft
tokens, $\alpha$, and the draft KV-read ratio, $s$, to throughput relative to
autoregressive (AR) decoding. We evaluate the resulting analytic surface and
place observed operating points on it. Measured component costs and paired
runtime observations determine the available cost anchors; assumptions about
unmeasured costs determine the extrapolation between operating points.

\subsection{From token progress to a normalized cost surface}
\label{sec:estimated-speedup-formulation}

Fix the model, hardware, execution state, and draft length $k$. Let $L$ be the
accepted prefix length in a complete speculative round. With one correction
or bonus token per round, the expected progress per request is
\begin{equation}
  \alpha = \frac{\mathbb{E}[L]}{k},
  \qquad
  \tau = 1+\mathbb{E}[L] = 1+k\alpha.
  \label{eq:estimated-speedup-progress}
\end{equation}
This expression does not require independent acceptance across draft
positions. If an AR iteration costs $T_p$ and a speculative round-equivalent
costs $C$, their throughput ratio at equal output progress is
$\eta=\tau T_p/C$. Comparing individual scheduler-iteration times would omit
the difference in committed output progress.

Write $G=T_{\mathrm{GEMM}}(B)$ and $A=T_{\mathrm{Attn}}(M)$, where $B$ is the
active request count and $M$ is the live KV volume. The ideal decomposition
uses $T_p=G+A$, linear attention cost in the KV-read volume, and shared KV
reads across a short verification block. When requests are evenly distributed
across the $k$ draft stages and one verification stage, define
\begin{equation}
  c_k=\frac{2k+1}{k+1},\qquad
  \rho=\frac{A}{G+A},\qquad
  g_k=\frac{T_{\mathrm{GEMM}}(c_kB)}{T_{\mathrm{GEMM}}(B)}.
  \label{eq:estimated-speedup-components}
\end{equation}
The balanced round-equivalent cost is
$C_{\mathrm{bal}}=(k+1)g_kG+(1+ks)A$. Normalizing by the AR cost yields
\begin{equation}
  D_0(s)=(k+1)g_k(1-\rho)+(1+ks)\rho,
  \qquad
  \eta_0(\alpha,s)=\frac{1+k\alpha}{D_0(s)}.
  \label{eq:estimated-speedup-ideal}
\end{equation}
Evaluating Eq.~\eqref{eq:estimated-speedup-ideal} over a grid produces the
surface; no free two-dimensional interpolant is fitted to the observations.
The $1\times$ contour has a direct interpretation:
\begin{equation}
  \eta_0>1
  \quad\Longleftrightarrow\quad
  \alpha>\frac{D_0(s)-1}{k}.
  \label{eq:estimated-speedup-boundary}
\end{equation}
At fixed costs, increasing acceptance increases useful progress, whereas
increasing the draft KV-read ratio increases cost. These are conditional
directions: changing the budget in an actual run also changes acceptance,
so the attainable operating points follow a workload-dependent trajectory
$\alpha(s)$ through the surface.

\subsection{Measurement definitions and cost anchors}
\label{sec:estimated-speedup-measurements}

We distinguish the configured budget $s_{\mathrm{cfg}}$ from the effective
logical KV-read ratio $s_{\mathrm{eff}}$. Minimum budgets, rounding, and
draft-token appends can make them differ. Where scheduler states expose
logical reads, we compute $s_{\mathrm{eff}}$ by dividing aggregate sparse
reads by the corresponding full logical KV volume of draft requests.
For variable-length rollouts without these counters, points use their
measured configuration $s_{\mathrm{cfg}}$. Neither quantity is a direct
measurement of HBM traffic or sparse-attention time.

For Qwen3-8B on two H100 GPUs with TP=2, the AR component profile at
$(B,S)=(64,8192)$ gives $A=13.1067$ ms and $G=3.2080$ ms per iteration per
rank. Here $G$ includes FFN, QKVO projections, and the LM head; other kernels
and TP collectives are outside this two-component denominator. Thus
$\rho=0.80337$. With $k=6$, the ideal mixed query count is
$c_kB=118.86$. Interpolating between pure-AR GEMM measurements at query
counts 64 and 128 gives $g_k=1.03608$. This interpolation is a proxy for
mixed-stage query scaling. Its interpolation anchors are measured at
$S=4096$, and the estimated ratio is transferred to $S=8192$ under the
approximation that projection scaling is
primarily determined by query count.

These values specify the original 8B surface. For example,
$(\alpha,s)=(0.8,0.05)$ gives an ideal estimate of $2.35\times$. This value
inherits the balanced scheduling and component-cost assumptions; it is not
an observed rollout speedup.

\subsection{Calibrating the 8B surface to scheduler windows}
\label{sec:estimated-speedup-calibration-8b}

We reconstruct paired decode windows from unprofiled AR and sparse runs.
Both endpoints have the same request set, KV progress, and verification
phase. With no admissions, completions, or capacity events inside the
window, the change in logical KV volume between these phases estimates
committed progress. We sum the CPU scheduler intervals within each TP rank
and take the larger rank total for each method. The ratio of these totals
at equal progress is a scheduler-window speedup estimate. It includes
exposed stalls but does not independently measure synchronized GPU wall
time or the final GPU drain.

For $B=64$, three paired windows span contexts 8247--8394 and 21 complete
rounds, implying $\tau_*=7$ and $\alpha_*=1$. Their effective draft-read
ratio is $s_*=0.050458$ and their speedup estimates are
$1.6748\times$, $1.6114\times$, and $1.6162\times$. The ideal surface gives
$2.8309\times$ at this coordinate. We calibrate an aggregate normalized
cost correction to the median window estimate $\widehat\eta_*$:
\begin{equation}
  D_* = \frac{1+k\alpha_*}{\widehat\eta_*},\qquad
  \Delta D=D_*-D_0(s_*),\qquad
  \widehat\eta_{\lambda}(\alpha,s)
  =\frac{1+k\alpha}{D_0(s)+\lambda\Delta D}.
  \label{eq:estimated-speedup-calibration}
\end{equation}
Here $D_*=4.33118$ and $\Delta D=1.85849$. The choice $\lambda=0$ recovers
the ideal surface and $\lambda=1$ passes through the calibration anchor.
Larger $\lambda$ values are additional cost scenarios, not confidence bounds.
At $(0.8,0.05)$, the calibrated estimate becomes $1.34\times$ and the
break-even acceptance increases from 0.245 to 0.555.

The size of the correction reflects a substantive execution difference.
The measured workload synchronizes requests into six all-draft iterations,
one all-verify iteration, and one stall. In the repeat corresponding to the
median speedup, these stages total 33.588, 21.254, and 22.681 ms per round,
respectively. The matched AR cost is 17.899 ms per iteration, giving
\begin{equation}
  \widehat\eta_*
  =\frac{7\cdot17.899}{33.588+21.254+22.681}
  \simeq1.616.
  \label{eq:estimated-speedup-window-example}
\end{equation}
Stall intervals account for 29.3\% of this measured round. They may expose
unfinished asynchronous verification work and cannot simply be removed
from the latency accounting. Synchronized verification also processes
$7B=448$ queries, exceeding the configured CUDA Graph capture limit of
160 and taking the eager path. Together with the difference between
GPU component sums and CPU interval timing, these effects explain why
$\Delta D$ must be interpreted as an aggregate correction rather than
a separately measured CPU overhead. Its individual causes are not
identified by this calibration.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/supporting_systems/estimated_speed_up/fig_alpha_s_speedup_calibration_comparison.pdf}
  \caption{Qwen3-8B ideal and scheduler-window-calibrated surfaces with a
  shared color scale. Brown diamonds show the window estimate used for
  calibration. Purple squares show a separate paired Offload/AR
  rollout comparison at nominal budget 0.03; its variable batch/context
  and generation-time denominator differ from the local window model.
  Gray circles are 12 measured checkpoint acceptance values at nominal
  budget 0.05, without matched AR speedups. Callouts distinguish
  runtime-derived speedups from surface estimates.}
  \label{fig:estimated-speedup-8b}
\end{figure}

Figure~\ref{fig:estimated-speedup-8b} also includes a paired three-step
8B rollout reference: Offload achieves $1.4909\times$ the AR
output throughput at $s_{\mathrm{cfg}}=0.03$ and acceptance proxy
0.77077. Substitution into the fixed-state surfaces gives $2.3692\times$
before calibration and $1.3289\times$ after calibration. The latter is
10.9\% below the observed ratio, but the workload and timing scopes differ;
this is a cross-workload comparison, not a matched-state prediction error.

\subsection{A rollout-calibrated surface for 1.7B}
\label{sec:estimated-speedup-calibration-17b}

The available 1.7B data provide paired rollout measurements but no matching
component profile or budget sweep. We therefore calibrate its own effective
cost scale from four post-warmup Offload/AR step pairs. Each step
uses 4096 requests across four TP=2 replicas; paired methods receive
identical global prompts. Actual batch and context lengths vary throughout
generation. Let $Y_{m,j}$ and $T_{m,j}$ denote output tokens and generation
wall time for method $m$ and step $j$. The aggregate speedup is
\begin{equation}
  \eta_*^{1.7}
  =\frac{\sum_jY_{\mathrm{Offload},j}/\sum_jT_{\mathrm{Offload},j}}
         {\sum_jY_{\mathrm{AR},j}/\sum_jT_{\mathrm{AR},j}}
  =\frac{49719.27}{31912.11}=1.55801.
  \label{eq:estimated-speedup-rollout-ratio}
\end{equation}
This ratio accounts for the different realized output lengths. We obtain
the acceptance proxy from the sum of accepted speculative tokens divided
by the sum of proposed speculative tokens over all steps and replicas,
giving $\alpha_*=0.756863$. This counter ratio approximates
Eq.~\eqref{eq:estimated-speedup-progress}; partial rounds and truncation
are not independently corrected by a complete-round counter here.

We retain the linear budget-cost form and calibrate its intercept:
\begin{equation}
  D_*^{1.7}=\frac{1+6\alpha_*}{\eta_*^{1.7}}=3.55658,
  \qquad
  \widehat\eta_{1.7}(\alpha,s_{\mathrm{cfg}})
  =\frac{1+6\alpha}{D_*^{1.7}+\beta(s_{\mathrm{cfg}}-0.03)}.
  \label{eq:estimated-speedup-17b}
\end{equation}
The parameter $D_*^{1.7}$ is an effective rollout cost scale, not a measured
local round latency. We do not transfer the 8B component costs or its
window correction into this estimate.

The slope $\beta$ remains unmeasured. The ideal normalized decomposition
suggests a slope of the form $k\rho$; we examine the assumed scenarios
$\beta\in\{3,4.5,6\}$ and display $\beta=6$. For budgets at least 0.03,
this choice gives the lowest speedups among these scenarios. It is not
an empirical lower bound or evidence that the 1.7B attention fraction
equals one. All three scenarios agree at the calibration budget, so
the present observations cannot select among them. At $\alpha=0.8$ and
$s_{\mathrm{cfg}}=0.20$, their estimates range from $1.43\times$ to
$1.27\times$, illustrating the uncertainty away from the anchor.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.82\linewidth]{figures/supporting_systems/estimated_speed_up/fig_alpha_s_speedup_1_7b.pdf}
  \caption{Qwen3-1.7B conditional surface calibrated to paired rollout
  throughput. Purple squares mark four measured step coordinates and
  the filled diamond is their aggregate anchor. The inset shows their
  individual runtime speedups and the surface estimates. Gray circles
  are 19 measured checkpoint acceptance values under a separate workload;
  no paired AR speedups are available for these checkpoints. The budget
  slope is assumed, and all four paired steps calibrate the displayed
  surface.}
  \label{fig:estimated-speedup-17b}
\end{figure}

\begin{table}[t]
  \centering
  \small
  \begin{tabular}{ccrrr}
    \toprule
    Paired step & Acceptance proxy & Runtime speedup & Surface estimate & Relative error \\
    \midrule
    1 & 0.754397 & $1.5825\times$ & $1.5538\times$ & $-1.81\%$ \\
    2 & 0.757266 & $1.4921\times$ & $1.5587\times$ & $+4.46\%$ \\
    3 & 0.759237 & $1.5461\times$ & $1.5620\times$ & $+1.03\%$ \\
    4 & 0.756635 & $1.6145\times$ & $1.5576\times$ & $-3.52\%$ \\
    \bottomrule
  \end{tabular}
  \caption{Measured 1.7B step ratios and estimates using the aggregate
  calibration. Relative error is $100(\widehat\eta/\eta_{\mathrm{runtime}}-1)$.
  All four steps have nominal budget 0.03 and belong to one training
  sequence; these are within-sample residuals, not independent validation.}
  \label{tab:estimated-speedup-17b-fit}
\end{table}

The displayed calibration has a mean absolute relative residual of 2.71\%
over the four steps (Table~\ref{tab:estimated-speedup-17b-fit}). Recalibrating
on three steps and predicting the remaining step gives a leave-one-step-out
mean absolute relative deviation of 3.60\%. This measures stability within
the same short sequence at one budget. It provides no validation of the
budget slope, and the steps are not independent random-seed replicates.

\subsection{Interpretation and limits of the estimates}
\label{sec:estimated-speedup-interpretation}

The surfaces express the mechanism targeted by Self-Sparse: reducing draft
KV reads lowers speculative cost while accepted prefixes amortize dense
projection and full-attention verification work. The $1\times$ contour
makes the resulting acceptance requirement explicit. The 1.7B paired
measurements establish actual rollout gains of $1.49$--$1.61\times$ in
their measured setting; the surface explains a conditional trade-off around
that operating region.

The checkpoint sweeps add measured acceptance coordinates, not extra
speedup measurements. We retain all 12 complete 8B checkpoint evaluations
and all 19 complete 1.7B evaluations in the calibrated figures. Their
respective acceptance ranges are 0.75754--0.82268 and 0.74418--0.78798,
at nominal budget 0.05. Position-level acceptance probabilities are used
to recover one prefix-fraction estimate per run; they are not separate
two-dimensional observations. A sweep across checkpoints at one budget
does not identify the acceptance--budget relationship or an optimal budget.

Calibration agreement must also be interpreted according to its scope.
The 8B anchor is reused to determine its cost correction, while the 1.7B
anchor aggregates the same steps whose residuals are reported. Their
different timing boundaries preclude using these residuals to claim that
one model size has a more accurate predictive surface. In both models,
the extrapolation holds effective cost parameters fixed as acceptance
and budget vary; actual rejection, kernel, and scheduling costs may change.
Testing those dependencies requires held-out budget values, direct committed
token counts, matched execution states, and timing that covers completed
GPU work. The current figures provide empirically anchored conditional
estimates of the acceleration regime under explicitly stated assumptions.


==> figs/sys_profiling/supporting_systems_final.tex <==
% Include this file from the paper directory. All four plotting regions are equal squares.
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{figures/supporting_systems/final/fig_supporting_systems_row.pdf}
  \caption{Systems motivation for sparse self-speculation and the KV-aware AIMD scheduler.
  From left to right: (1) Qwen3-8B full-AR GPU kernel durations in milliseconds per iteration per
  TP rank on two H100 GPUs, excluding TP collectives. Five attention-dominated
  configurations have $B S=512K$ nominal live-KV tokens, with $K=1024$.
  QKVO includes QKV/output projections; Other groups the remaining non-collective
  kernels. (2) Response-length survival distribution for 4096 requests in a
  Qwen3-1.7B rollout with fixed Offload-256. (3) Active-request counts and cached
  KV utilization from the same rollout's four replicas. Color indicates local
  scheduler iteration divided by each replica's total iterations. Horizontal
  jitter is at most three requests and affects display only. The purple circle
  and text indicate the tail crossing where utilization falls below 70\%
  at approximately 68\% scheduler progress on average (64.6--70.3\% across
  replicas). Each estimate linearly interpolates the final
  downward threshold crossing between adjacent sampled states.
  (4) Cumulative rebuilding demand and D2H-plus-H2D movement over four successive
  Qwen3-1.7B RL steps. Recompute event timing and sizes are simulated, constrained
  by observed per-replica step totals, retraction counts, and KV pressure;
  Offload and KV-aware AIMD scheduler movement traces are recorded. Steps are
  concatenated separately for each method using the maximum replica iteration
  count. Rebuilding and
  moving a page need not have equal execution cost. The panels show component
  costs and observed operating states, without isolating the causal effect of
  response-length variability or measuring recomputation timing.}
  \label{fig:supporting-systems-final}
\end{figure}


==> figs/why_ssrl_2/tables/budget_results.tex <==
\begin{tabular}{llrrrrrr}
\toprule
Budget & Split & $\alpha_{1.7}$ & Meas. & Est. & $\alpha_{8}$ & Meas. & Est. \\
\midrule
0.03 & Calibration & 0.754 & 1.469 & 1.511 & 0.756 & 1.307 & 1.330 \\
0.05 & Held-out & 0.795 & 1.533 & 1.533 & 0.804 & 1.370 & 1.367 \\
0.10 & Calibration & 0.854 & 1.516 & 1.519 & 0.847 & 1.358 & 1.352 \\
0.20 & Held-out & 0.903 & 1.414 & 1.402 & 0.912 & 1.311 & 1.299 \\
0.35 & Calibration & 0.937 & 1.242 & 1.229 & 0.943 & 1.179 & 1.167 \\
0.50 & Calibration & 0.958 & 1.094 & 1.088 & 0.967 & 1.058 & 1.059 \\
\bottomrule
\end{tabular}


==> figs/why_ssrl_2/tables/fit_summary.tex <==
\begin{tabular}{lrrrrrr}
\toprule
Configuration & $\rho$ & $g_k$ & $\delta$ & Ideal MAPE & Cal. MAPE & Cal. max. \\
\midrule
1.7B & 0.904 & 1.041 & 1.886 & 84.61 & 0.80 & 1.91 \\
8B (control) & 0.803 & 1.036 & 1.885 & 67.37 & 0.61 & 0.88 \\
8B & 0.803 & 1.036 & 1.787 & 63.03 & 0.68 & 1.09 \\
\bottomrule
\end{tabular}


==> figs/why_ssrl_2/tables/rl_steps.tex <==
\begin{tabular}{llrrrr}
\toprule
Model & RL step & $\alpha_{\rm log}$ & Measured & Estimated & Diff. (\%) \\
\midrule
1.7B & Step a & 0.7544 & 1.583 & 1.514 & -4.35 \\
1.7B & Step b & 0.7573 & 1.492 & 1.518 & +1.76 \\
1.7B & Step c & 0.7566 & 1.614 & 1.517 & -6.02 \\
1.7B & Step d & 0.7592 & 1.546 & 1.522 & -1.59 \\
8B & Step a & 0.7724 & 1.468 & 1.354 & -7.73 \\
8B & Step b & 0.7731 & 1.500 & 1.355 & -9.64 \\
8B & Step c & 0.7668 & 1.505 & 1.346 & -10.58 \\
\bottomrule
\end{tabular}


==> figs/why_ssrl_2/tables/rl_transfer.tex <==
\begin{tabular}{lrrrrrr}
\toprule
Local surface & RL steps & $\alpha_{\rm log}$ & Meas. & Est. & Diff. (\%) & Step MAPE \\
\midrule
1.7B & 4 & 0.757 & 1.558 & 1.518 & -2.59 & 3.43 \\
8B (control) & 3 & 0.771 & 1.491 & 1.321 & -11.41 & 11.40 \\
8B & 3 & 0.771 & 1.491 & 1.352 & -9.32 & 9.31 \\
\bottomrule
\end{tabular}


==> figs/why_ssrl_2/tables/state_diagnostics.tex <==
\begin{tabular}{lrrrr}
\toprule
Configuration & $B$ & $S$ & $\alpha$ & Measured speedup \\
\midrule
1.7B & 32 & 8K & 0.784 & 1.227 \\
1.7B & 64 & 4K & 0.730 & 1.102 \\
1.7B & 32 & 16K & 0.855 & 1.707 \\
8B (control) & 32 & 8K & 0.790 & 1.121 \\
8B (control) & 64 & 4K & 0.766 & 1.030 \\
8B (control) & 32 & 16K & 0.891 & 1.525 \\
\bottomrule
\end{tabular}

